LLMs Improving LLMs: Agentic Discovery for Test-Time Scaling

Test-time scaling (TTS) has become an effective approach for improving large language model performance by allocating additional computation during inference. However, existing TTS strategies are largely hand-crafted: researchers manually design reasoning patterns and tune heuristics by intuition, leaving much of the computation-allocation space unexplored. We propose an environment-driven framework, AutoTTS, that changes what researchers design: from individual TTS heuristics to environments where TTS strategies can be discovered automatically. The key to AutoTTS lies in environment construction: the discovery environment must make the control space tractable and provide cheap, frequent feedback for TTS search. As a concrete instantiation, we formulate width--depth TTS as controller synthesis over pre-collected reasoning trajectories and probe signals, where controllers decide when to branch, continue, probe, prune, or stop and can be evaluated cheaply without repeated LLM calls. We further introduce beta parameterization to make the search tractable and fine-grained execution trace feedback to improve discovery efficiency by helping the agent diagnose why a TTS program fails. Experiments on mathematical reasoning benchmarks show that the discovered strategies improve the overall accuracy--cost tradeoff over strong manually designed baselines. The discovered strategies generalize to held-out benchmarks and model scales, while the entire discovery costs only $39.9 and 160 minutes. Our data, and code will be open-source at https://github.com/zhengkid/AutoTTS.

==> Fig/cost_efficiency.tex <==
\pgfplotsset{compat=1.18}
\definecolor{costblue}{HTML}{6BAED6}
\definecolor{timeorange}{HTML}{FDAE6B}
\definecolor{tracegreen}{HTML}{74C476}

\begin{figure}[t]
\centering
\begin{tikzpicture}
\begin{axis}[
    ybar,
    width=0.46\textwidth,
    height=0.28\textwidth,
    bar width=20pt,
    ymin=0,
    ymax=1.15,
    ylabel={Normalized value},
    symbolic x coords={Cost, Time, Trace},
    xtick=data,
    xticklabel style={font=\small},
    yticklabel style={font=\small},
    ylabel style={font=\small},
    nodes near coords={\pgfplotspointmeta},
    nodes near coords style={font=\footnotesize, yshift=2pt},
    enlarge x limits=0.35,
    ymajorgrids=true,
    major grid style={dashed, gray!25},
    axis line style={black!60},
    tick style={black!60},
]
\addplot[
    ybar,
    draw=costblue!80!black,
    fill=costblue!70,
    point meta=explicit symbolic
] coordinates {(Cost, 0.2485) [\$39.87]};

\addplot[
    ybar,
    draw=timeorange!80!black,
    fill=timeorange!75,
    point meta=explicit symbolic
] coordinates {(Time, 1.0000) [160.47 min]};

\addplot[
    ybar,
    draw=tracegreen!80!black,
    fill=tracegreen!70,
    point meta=explicit symbolic
] coordinates {(Trace, 0.0872) [14.0 GB]};
\end{axis}
\end{tikzpicture}
\caption{Summary of discovery overhead over five discovery rounds. Values are normalized by the largest quantity for visualization, while labels report the original measurements.}
\label{fig:discovery_overhead}
\end{figure}

==> Fig/overview_fig.tex <==
% =====================================================================
% figure_overview.tex
%
% Standalone TikZ snippet for the overview/teaser of the paper.
% Designed to be \input'd inside a figure environment in the main file.
%
% --------------------------- USAGE -----------------------------------
% In your MAIN preamble, make sure these are loaded:
%   \usepackage{tikz}
%   \usepackage{xcolor}
%   \usepackage{fontawesome5}     % \faBrain, \faDatabase, \faCog,
%                                 % \faMicrochip, \faFolderOpen, ...
%   \usepackage{amssymb}
%   \usetikzlibrary{positioning, arrows.meta, calc, fit,
%                   shapes.geometric, shapes.misc, shapes.callouts,
%                   backgrounds, decorations.pathreplacing}
%
% In the body of your MAIN file:
%   \begin{figure*}[t]                         % figure* spans both columns
%     \centering
%     \resizebox{\textwidth}{!}{\input{overview_fig}}
%     \caption{...}\label{fig:overview}
%   \end{figure*}
%
% Compile with lualatex / xelatex (recommended for fontawesome5 icons).
% =====================================================================

% ------------------- Color palette -----------------------------------
\providecolor{warmFill}{HTML}{FEF3C7}
\providecolor{warmBorder}{HTML}{D97706}
\providecolor{coolFill}{HTML}{DBEAFE}
\providecolor{coolBorder}{HTML}{2563EB}
\providecolor{coolDeep}{HTML}{1D4ED8}
\providecolor{midFill}{HTML}{F3F4F6}
\providecolor{midBorder}{HTML}{6B7280}
\providecolor{stageFill}{HTML}{EFF6FF}
\providecolor{stageBorder}{HTML}{2563EB}
\providecolor{arrowGray}{HTML}{374151}
\providecolor{textGray}{HTML}{6B7280}
\providecolor{proposerOrange}{HTML}{F59E0B}
\providecolor{fsFill}{HTML}{EDE9FE}
\providecolor{fsBorder}{HTML}{7C3AED}
\providecolor{tileFill}{HTML}{FFFFFF}
\providecolor{tileBorder}{HTML}{C4B5FD}
\providecolor{stopRed}{HTML}{DC2626}
\providecolor{logsFill}{HTML}{FEF3C7}
\providecolor{logsBorder}{HTML}{D97706}

% ------------------- Layout plan (cm) --------------------------------
%
%   Total drawing width  : ~17.1 cm  (intended for figure*)
%   Total drawing height : ~12.3 cm
%
%   Horizontal slots:
%       boxA     x =  0.00 ..  6.56     warm
%       cpu link x ~  7.43
%       boxB     x =  8.30 .. 12.36     mid
%       boxC     x = 13.00 .. 17.06     cool
%
%       fs       x =  0.00 ..  3.72     filesystem (violet)
%       brain    x ~  4.55              proposer
%       cand     x ~  5.65              candidate
%       stage    x =  7.10 .. 13.80     CENTER STAGE  (width 6.7)
%       logs     x = 14.71 .. 17.06
%
%   Vertical bands:
%       y = 9.95  top-row label (1)
%       y = 9.50  top of top-row boxes (anchor=NW)
%       y = 7.55  cpu/arrow midline
%       y = 5.50  divider
%       y = 5.15  bottom-row label (2)
%       y = 4.70  top of fs / stage
%       y = 4.30  Step ① and ② headers
%       y = 2.55  proposer + candidate row
%       y = 0.10  bottom of stage / fs
%       y = -1.20 feedback-curve apex with Step ③ badge
%       y = -2.10 footer
%
% ---------------------------------------------------------------------

\begin{tikzpicture}[
  font=\sffamily,
  >={Stealth[length=3mm,width=2mm]},
  warm/.style    ={rectangle, rounded corners=4pt, draw=warmBorder, fill=warmFill,
                   line width=1pt, inner sep=8pt, align=left},
  cool/.style    ={rectangle, rounded corners=4pt, draw=coolBorder, fill=coolFill,
                   line width=1pt, inner sep=8pt, align=left},
  midbox/.style  ={rectangle, rounded corners=4pt, draw=midBorder, fill=midFill,
                   line width=1pt, inner sep=8pt, align=left},
  fsbox/.style   ={rectangle, rounded corners=4pt, draw=fsBorder, fill=fsFill,
                   line width=1pt, inner sep=7pt, align=left},
  filetile/.style={rectangle, rounded corners=2pt, draw=tileBorder, fill=tileFill,
                   line width=0.6pt, inner sep=2pt, font=\scriptsize, align=center,
                   minimum width=1.4cm, minimum height=0.8cm},
  stage/.style   ={rectangle, rounded corners=8pt, draw=stageBorder, fill=stageFill,
                   line width=1.4pt, inner sep=10pt},
  ctrlbox/.style ={rectangle, rounded corners=4pt, draw=coolDeep, fill=white,
                   line width=1pt, inner sep=4pt, align=center, text width=1.9cm,
                   font=\small},
  envbox/.style  ={rectangle, rounded corners=4pt, draw=coolDeep, fill=white,
                   line width=1pt, minimum width=2.5cm, minimum height=2.4cm},
  candbox/.style ={rectangle, rounded corners=3pt, draw=arrowGray, fill=white,
                   line width=0.8pt, inner sep=4pt, font=\small\bfseries},
  pill/.style    ={rectangle, rounded corners=6pt, draw=coolBorder, fill=white,
                   line width=0.7pt, inner sep=3pt, font=\tiny},
  stepbadge/.style={rectangle, rounded corners=3pt, draw=none, font=\small\bfseries,
                    inner sep=2pt, align=left},
  logsbox/.style ={rectangle, rounded corners=4pt, draw=logsBorder, fill=logsFill!40,
                   line width=1pt, inner sep=5pt, font=\scriptsize, align=left},
  arrow/.style   ={->, draw=arrowGray, line width=1pt},
  thickarrow/.style={->, draw=arrowGray, line width=1.4pt},
  faded/.style   ={->, dashed, draw=textGray, line width=0.7pt},
  figcap/.style  ={font=\scriptsize\itshape, color=textGray},
]

% =====================================================================
% TOP ROW : Environment Construction
% =====================================================================
\node[anchor=west, font=\bfseries, color=coolDeep] (toplab) at (0,9.95) {TOP ROW:};
\node[anchor=west, font=\bfseries] at (toplab.east) [xshift=2mm]
  {\textcircled{1}~Environment Construction};

% --- Box A : warm, structured bullets
\node[warm, text width=6.3cm, anchor=north west, minimum height=3.85cm] (boxA)
  at (0,9.50) {%
  \textbf{Define online reasoning environment $E$}\\[5pt]
  \footnotesize
  $\bullet$~\textbf{action space:}\\
  \mbox{\phantom{$\bullet$~}}branch / continue / probe / prune / stop\\[2pt]
  $\bullet$~\textbf{observation:}\\
  \mbox{\phantom{$\bullet$~}}progress + probe answers + remaining budget\\[2pt]
  $\bullet$~\textbf{cost / reward model}\\[6pt]
  \mbox{}\hfill{\scriptsize\itshape\color{textGray}human-engineered}
};

% --- CPU + label between Box A and Box B
%     Explicit text width prevents the longest line ("base-reasoner")
%     from being hyphen-broken when the figure is rescaled.
\node[font=\Large, anchor=center] (cpu) at (7.50,7.55) {\faMicrochip};
\node[anchor=north, font=\scriptsize\bfseries, align=center, text width=2.2cm,
      inner sep=1pt]
  at (cpu.south) [yshift=-0.5mm]
  {one-time\\ base-reasoner\\ rollout};

% --- Box B : trace bundles (short title + icon, fits one line)
\node[midbox, text width=3.8cm, anchor=north west, minimum height=3.85cm] (boxB)
  at (8.10,9.50) {%
  {\bfseries Trace bundles}~\faDatabase\\[5pt]
  \footnotesize multi-trajectory rollouts\\
  + intermediate probes
};

% --- Box C : replay environment (short title + icon, fits one line)
\node[cool, text width=3.8cm, anchor=north west, minimum height=3.85cm] (boxC)
  at (12.80,9.50) {%
  {\bfseries Replay env $\widehat{E}$}~\faCog\\[5pt]
  \footnotesize deterministic simulation;\\mirrors $E$
};

% --- Top-row arrows (drawn at the cpu midline so labels stay centered)
\draw[thickarrow] (boxA.east|-cpu) -- ($(cpu.west)+(-1mm,0)$);
\draw[thickarrow] ($(cpu.east)+(1mm,0)$) -- (boxB.west|-cpu);
\draw[thickarrow] (boxB.east) -- (boxC.west);

% =====================================================================
% Divider
% =====================================================================
\draw[dashed, textGray, line width=0.5pt] (-0.4,5.50) -- (17.2,5.50);

% =====================================================================
% BOTTOM ROW : Discovery Loop
% =====================================================================
\node[anchor=west, font=\bfseries, color=coolDeep] (botlab) at (0,5.15) {BOTTOM ROW:};
\node[anchor=west, font=\bfseries] at (botlab.east) [xshift=2mm]
  {\textcircled{2}~Automatic Discovery Loop over Replay Environment};
\node[anchor=east, figcap] at (17.2,5.15) {filesystem stores all attempts};

% =====================================================================
% Filesystem D (left)
%
% Implemented as an empty container + absolutely positioned children,
% so the title does not get vertically centred inside the over-tall box.
% =====================================================================
\node[fsbox, minimum width=4.0cm, minimum height=4.30cm, anchor=north west,
      inner sep=0pt] (fs) at (0,4.70) {};

% Title and subtitle, anchored to fs.north west
\node[anchor=north west, inner sep=0pt]
  at ($(fs.north west)+(2.5mm,-3mm)$)
  {\faFolderOpen~{\bfseries Filesystem $\mathcal{D}$}};
\node[anchor=north west, inner sep=0pt, font=\footnotesize, color=textGray]
  at ($(fs.north west)+(2.5mm,-9mm)$)
  {all experience};

% File tiles 2x2 inside fs
\node[filetile, anchor=center] at ($(fs.north west)+(1.20,-2.05)$)
  {$(f_1,\beta_1)$\\\faMedal};
\node[filetile, anchor=center] at ($(fs.north west)+(2.75,-2.05)$)
  {$(f_2,\beta_2)$\\\faMedal};
\node[filetile, anchor=center] at ($(fs.north west)+(1.20,-3.15)$)
  {$(f_3,\beta_3)$\\\faMedal};
\node[filetile, anchor=center] at ($(fs.north west)+(2.75,-3.15)$)
  {$(f_4,\beta_4)$\\\faMedal};

\node[figcap, anchor=south, inner sep=0pt]
  at (fs.south) [yshift=2.5mm] {config + actions + score};

% =====================================================================
% Step 1 : Propose
% =====================================================================
% Step badge sits in the same horizontal band (y=4.30) as the Step-2 header
% inside the stage, so the two badges read as a row.
\node[stepbadge, anchor=center] at (5.10,4.30)
  {\textcircled{1}~Propose};

% Brain proposer
\node[circle, draw=proposerOrange, fill=proposerOrange!30, line width=1pt,
      minimum size=1.2cm] (prop) at (5.10,2.55) {\Large\faBrain};
\node[font=\scriptsize, anchor=north] at (prop.south) [yshift=-0.5mm] {proposer};

% Speech bubble pointing down to prop, placed clearly between the Step-1
% badge (at y=4.30) and the brain top (at y=3.15).
\node[ellipse callout, callout absolute pointer={(prop.north)},
      callout pointer width=2mm, callout pointer shorten=0pt,
      draw=textGray, fill=white, line width=0.6pt, font=\tiny, inner sep=2pt,
      anchor=center, align=center] at (5.10,3.65)
  {push the\\frontier outward};

% Candidate (the "(f,beta)" box is self-descriptive; no extra caption)
\node[candbox, anchor=west] (cand) at (6.20,2.55) {$(f,\beta)$};

% Wiring: fs -> prop -> cand
\draw[faded] (fs.east|-prop) --
  node[above, font=\tiny, inner sep=1pt] {read history} (prop.west);
\draw[arrow] (prop.east) -- (cand.west);

% =====================================================================
% Step 2 : Center Stage (inner episode loop)
% =====================================================================
\node[stage, minimum width=6.7cm, minimum height=4.60cm, anchor=north west]
  (stage) at (7.10,4.70) {};

% Step ② header inside stage at top-left  (kept short so it does not
% collide with the ×T pill on the right)
\node[anchor=north west, font=\bfseries] (s2hdr)
  at (stage.north west) [shift={(3mm,-3mm)}]
  {\textcircled{2}~Interact (inner loop)};
\node[anchor=north west, font=\tiny\bfseries, color=coolDeep, inner sep=0pt]
  at (s2hdr.south west) [yshift=-0.5mm]
  {CENTER STAGE};

% ×T pill at top-right of stage (compact form to avoid colliding with the
% "Replay env" header that sits just below it)
\node[pill, anchor=north east] at (stage.north east) [shift={(-3mm,-3mm)}]
  {$\circlearrowright\,\times T$ steps};

% --- Controller box (left half)  -- absolute coordinates ---
\node[ctrlbox, anchor=center] (ctrl) at (8.45,2.50) {%
  \textbf{Controller}\\[2pt]
  \footnotesize $\pi_{f,\beta}$\\
  \footnotesize $=\pi_{f,g_f(\beta)}$
};

% --- Replay env mini box (right half)  -- absolute coordinates ---
%     Header sits just above the box.  The xT-steps pill in the stage's NE
%     corner has been compacted so the two no longer overlap horizontally.
\node[envbox, anchor=center] (env) at (12.25,2.50) {};
\node[anchor=south, font=\scriptsize\bfseries, color=coolDeep, inner sep=1pt]
  at (env.north) [yshift=0.5mm]
  {Replay env $\widehat{E}$};

% --- Inside env: trajectories ---
\coordinate (eo) at ($(env.south west)+(4mm,4mm)$);
% main (continued) trajectory
\draw[coolBorder, line width=1pt] (eo)++(0.55,0) -- ++(0,1.55);
\fill[coolBorder] (eo)++(0.55,0.40) circle (1.1pt);
\fill[coolBorder] (eo)++(0.55,0.85) circle (1.1pt);
\fill[coolBorder] (eo)++(0.55,1.30) circle (1.1pt);
% branch
\draw[coolBorder, line width=1pt] (eo)++(0.55,0.55) -- ++(0.55,0.45);
\fill[coolBorder] (eo)++(1.10,1.00) circle (1.1pt);
\node[anchor=west, font=\tiny\bfseries, color=coolBorder, inner sep=1pt]
  at ($(eo)+(1.00,0.80)$) {branch};
% stop on top of main trajectory
\fill[stopRed] (eo)++(0.55,1.55) circle (1.4pt);
\node[anchor=west, font=\tiny\bfseries, color=stopRed, inner sep=1pt]
  at ($(eo)+(0.65,1.65)$) {stop};
% pruned trajectory (dashed with x markers)
\draw[gray!50, dashed, line width=0.6pt] (eo)++(1.55,0) -- ++(0,0.55);
\draw[gray!60, line width=0.7pt] (eo)++(1.50,0.50) -- ++(0.10,0.10);
\draw[gray!60, line width=0.7pt] (eo)++(1.50,0.60) -- ++(0.10,-0.10);
\node[anchor=center, font=\tiny\itshape, color=textGray, inner sep=0pt]
  at ($(eo)+(1.55,0.25)$) {pruned};
% axes
\draw[->, gray!70, line width=0.4pt] (eo) -- ++(1.80,0)
  node[right=-1pt, font=\tiny, gray] {w};
\draw[->, gray!70, line width=0.4pt] (eo) -- ++(0,1.80)
  node[above=-1pt, font=\tiny, gray] {d};

% --- Action / state arrows between Controller and Env ---
% Action arrow (top of band) -- only the bold "action a_t"
\draw[arrow] ($(ctrl.east)+(0,4mm)$) -- ($(env.west)+(0,4mm)$);
\node[font=\scriptsize\bfseries, anchor=south, inner sep=1pt]
  at ($($(ctrl.east)!0.5!(env.west)$)+(0,4.5mm)$) {action $a_t$};

% State arrow (bottom of band)
\draw[arrow] ($(env.west)+(0,-4mm)$) -- ($(ctrl.east)+(0,-4mm)$);
\node[font=\scriptsize, anchor=north, align=center, inner sep=1pt]
  at ($($(env.west)!0.5!(ctrl.east)$)+(0,-4.5mm)$)
  {next state $s_{t+1}$\\+ cost $c_t$};

% Caption inside stage at bottom (lifted higher to avoid the Step-3 badge)
\node[anchor=south, font=\scriptsize\itshape, color=textGray,
      text width=6.5cm, align=center]
  at (stage.south) [yshift=8mm]
  {episode terminates on stop or budget exhaustion};

% =====================================================================
% Logs / Score (right)
% =====================================================================
\node[font=\scriptsize\itshape, color=textGray, anchor=south]
  at (15.85,4.40) {logs of this attempt};
\node[logsbox, anchor=north east, text width=2.0cm] (logs) at (17.05,4.35) {%
  \faCode~~config $(f,\beta)$\\[2pt]
  \faScroll~~actions log\\[2pt]
  \faMedal~~$\widehat{J}_{\mathrm{acc}},~\widehat{J}_{\mathrm{cost}}$
};

% Arrow stage -> logs
\draw[thickarrow] (stage.east|-logs.west) -- (logs.west);

% =====================================================================
% Step 3 : feedback curve (logs -> fs) with badge label at midpoint
% =====================================================================
\draw[thickarrow, line width=1.2pt]
  (logs.south) .. controls +(0,-2.6) and +(0,-2.6) ..
  node[stepbadge, fill=white, font=\bfseries, midway, inner sep=4pt]
       {\textcircled{3}~Store all logs to $\mathcal{D}$}
  (fs.south);

% =====================================================================
% Footer
% =====================================================================
\node[anchor=north, font=\scriptsize\itshape, color=textGray, text width=16cm,
      align=center] at (8.55,-2.10)
  {The base reasoning model is called only during trace generation;
   candidate evaluation is fully replayed in $\widehat{E}$.};

\end{tikzpicture}

